Magic Quantum Code Surgery

Non-Clifford operations required for universal quantum computation can be implemented by measuring logical Clifford operators. We present a generalized framework to fault-tolerantly measure transversal Clifford logical operators in quantum low-density parity check (QLDPC) codes. Our protocol takes any QLDPC code and deforms the code across additional ancillary qubits such that a product of stabilizers measures the desired logical Clifford operator. We prove that the deformed, Clifford-stabilized code remains LDPC and that its distance is preserved up to a constant factor independent of the number of physical qubits. We further prove that the Clifford measurement has a fault distance against data qubit and measurement errors that grows linearly with the distance of the original code. We apply our methods to implement logical non-Clifford gates in algorithmically relevant subroutines and to prepare magic states in quantum stabilizer codes.

==> preamble.tex <==
\makeatletter
\@ifclassloaded{revtex4-2}{}{\usepackage[margin=1in]{geometry}}
\makeatother
\usepackage{amsmath,amsthm,amsfonts,amssymb,mathrsfs}
\usepackage{graphicx}
\usepackage{cancel}
\usepackage{bm}
\usepackage{tikz}
\usepackage{csquotes}
\usepackage{tikz-3dplot}
\usepackage{physics}
\usepackage{dsfont}
\usepackage{float}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{tcolorbox}
\makeatletter
\@ifclassloaded{revtex4-2}{\let\affil\affiliation
}{\usepackage{authblk}}
\makeatother

\tcbuselibrary{breakable}
\usepackage{keytheorems}
\newkeytheorem{definition}[parent=section, tcolorbox-no-titlebar={breakable, colback=blue!10}]
\newkeytheorem{example,lemma,conjecture,claim,theorem,proposition,corollary,fact,assumption,construction}[sibling=definition, tcolorbox-no-titlebar={breakable, colback=blue!10}]
\theoremstyle{definition}
\newtheorem{protocol}{Protocol}[section]

\newkeytheorem{remark}[parent=section, tcolorbox-no-titlebar={breakable}]
\allowdisplaybreaks[4]
\interdisplaylinepenalty=0
\makeatletter
\renewcommand{\log}{\mathop{\operator@font log}\nolimits}
\makeatother
\IfFileExists{bbm.sty}{\usepackage{bbm}}{\providecommand{\mathbbm}{\mathds}}
\usepackage{stmaryrd}
\usepackage{braket}
\makeatletter
\@ifpackageloaded{natbib}{}{\usepackage[numbers,sort&compress]{natbib}}
\makeatother
\usepackage{hyperref}
\usepackage[ruled,noline,longend]{algorithm2e}
\SetAlgoNoLine
\AtBeginDocument{\SetAlgoNoLine}
\SetAlgoLongEnd
\RestyleAlgo{boxruled}
\LinesNumbered
\definecolor{algcommentgray}{gray}{0.35}
\newcommand{\AlgCommentFont}[1]{\textcolor{algcommentgray}{#1}}
\SetCommentSty{AlgCommentFont}
\SetKwComment{tcp}{{\color{algcommentgray}$\blacktriangleright$}\ }{}
\usepackage{tcolorbox}
\tcbuselibrary{breakable}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.85}
\setcounter{topnumber}{3}
\setcounter{totalnumber}{5}
\newenvironment{longalgorithm}[2][]{\begin{tcolorbox}[breakable, sharp corners, boxsep=0pt,
      boxrule=\algoheightrule, colframe=black, colback=white,
      left=18pt, right=4pt, top=5pt, bottom=5pt, #1]\refstepcounter{algocf}\noindent\hspace*{-14pt}{\textbf{\algorithmcfname~\thealgocf:} #2}\par
  \addcontentsline{loa}{algocf}{\protect\numberline{\thealgocf}#2}\par\nobreak\vspace{2pt}\nointerlineskip
  \moveleft18pt\vbox{\hrule width \dimexpr\linewidth+22pt\relax height \algoheightrule}\vspace{3pt}\setcounter{AlgoLine}{0}\RestyleAlgo{plain}}{\end{tcolorbox}}
\DontPrintSemicolon
\SetKwInput{KwIn}{Require}
\SetKwInput{KwOut}{Ensure}
\SetKwFor{For}{for}{do}{end for}
\SetKwFor{ForEach}{for each}{do}{end for}
\SetKwFor{While}{while}{do}{end while}
\makeatletter
\newenvironment{breakablealgorithm}{\par\addvspace{\intextsep}\hrule height .8pt\kern2pt
  \renewcommand{\caption}[2][]{\refstepcounter{algocf}\noindent\textbf{\algorithmcfname~\thealgocf:} ##2\par
    \kern2pt\hrule\kern2pt
    \ifx\relax##1\relax
      \addcontentsline{loa}{algocf}{\protect\numberline{\thealgocf}##2}\else
      \addcontentsline{loa}{algocf}{\protect\numberline{\thealgocf}##1}\fi
  }}{\par\kern2pt\hrule\addvspace{\intextsep}}
\makeatother
\usepackage{old-arrows}
\usepackage{color}
\usepackage{array, tabularx}
\usepackage{longtable}
\makeatletter
\@ifclassloaded{revtex4-2}{\appdef\@mkpream@relax{\let\@endpbox\relax}}{}
\makeatother
\usepackage{booktabs}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcommand{\Circo}[0]{\mathfrak{C}}
\newcommand{\restrict}[2]{#1 \vert_{#2}}
\newcommand{\physq}[0]{\mathcal{M}}


\newcommand{\Xp}[0]{\mathcal{X}}
\newcommand{\Zp}[0]{\mathcal{Z}}

\newcommand{\nS}[1]{\mathbb{N}_{#1}}
\newcommand{\aS}[1]{\mathbb{C}_{#1}}

\newcommand{\nD}[1]{D^N_{#1}}
\newcommand{\aD}[1]{D^C_{#1}}

\newcommand{\control}[3]{C_{#1} {#2}_{#3}}
\usetikzlibrary{3d, shapes, arrows.meta, decorations.pathreplacing, decorations.markings, cd, shapes.geometric, calc}
\IfFileExists{tikzlibrarycalligraphy.code.tex}{\usetikzlibrary{calligraphy}}{}
\pgfkeysifdefined{/pgf/decoration/calligraphic brace/.@cmd}{}{\pgfkeys{/pgf/decoration/calligraphic brace/.style={brace}}}
\tikzstyle{midarrow} = [decoration={markings, mark= at position 0.6 with {\arrow{Stealth}}}, postaction={decorate}]
\renewcommand{\comment}[1]{{\color{red} #1}}

\newcommand{\YR}[1]{{\color{Teal} [Collin: #1]}}

\newcommand{\kc}[1]{{\color{cyan} [Katie: #1]}}

\newcommand{\bb}[1]{{\color{purple}[BB: #1]}}




\newcommand{\vva}[1]{{\color{magenta} [VVA: #1]}}









\newcommand{\al}[1]{{\color{DarkGreen} [Ana: #1]}}

\newcommand{\hp}[1]{{\color{brown} [Harry: #1]}}

\newcommand{\NT}[1]{{\color{orange} [NT: #1]}}

\newcommand{\dom}[1]{\textcolor{blue}{[Dom: #1]}}

\newcommand{\todo}[1]{\textcolor{blue}{[TO-DO: #1]}}

\newcommand{\new}[1]{{\color{DarkMagenta}#1}}
\definecolor{FGreen}{RGB}{58,158,92}
\definecolor{lightred}{RGB}{223, 123, 84}
\definecolor{lightbrown}{RGB}{242,216,199}
\definecolor{invisiblegray}{RGB}{238,238,237}
\definecolor{lightgreen}{RGB}{222, 235, 218}
\definecolor{lightcyan}{RGB}{153, 191, 216}
\definecolor{lightcyan2}{RGB}{208, 224, 235}
\definecolor{cyan2}{RGB}{144,201,226}
\definecolor{lightyellow}{RGB}{252, 238, 183}
\definecolor{OrangeRed}{RGB}{223,123,84}
\definecolor{CyanGreen}{RGB}{81,177,184}
\definecolor{rose}{RGB}{226,45,139}
\definecolor{Ycolor}{RGB}{248,236,104}
\definecolor{Hcolor}{RGB}{255,255,0}
\definecolor{Xcolor}{RGB}{246,143,138}
\definecolor{Zcolor}{RGB}{210,254,206}
\definecolor{Lred}{RGB}{244,163,163}
\definecolor{Lgreen}{RGB}{160,211,179}
\definecolor{Lblue}{RGB}{170,183,240}
\definecolor{tickcolor}{RGB}{181,0,250}
\definecolor{DarkBlue}{RGB}{14,38,80}
\definecolor{greenblue}{RGB}{0,255,127}
\definecolor{darkblue}{RGB}{57,85,134}
\definecolor{electrored}{RGB}{244,96,85}
\definecolor{electrored2}{RGB}{245,107,94}
\definecolor{BBXcheck}{RGB}{210,234,206}
\definecolor{BBZcheck}{RGB}{204,204,250}
\definecolor{softred}{RGB}{245,206,206}
\definecolor{fuchsiapurple}{RGB}{180, 0, 255}
\definecolor{Teal}{RGB}{62,138,141}
\definecolor{gold}{RGB}{233,168,58}
\definecolor{Crimson}{RGB}{220,20,60}
\definecolor{RedOrange}{RGB}{255,69,0}
\definecolor{DarkMagenta}{RGB}{139,0,139}
\definecolor{DarkGreen}{RGB}{0,100,0}
\definecolor{MidnightBlue}{RGB}{25,25,112}



\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\renewcommand{\k}{\mathbf{k}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\Z}{\mathbb{Z}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\charge}{k}
\newcommand{\totalcharge}{K}
\newcommand{\B}{\mathbb{B}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\Ocal}{\mathcal{O}}
\renewcommand{\Vec}{\mathcal{V}ec}
\newcommand{\Rep}{\text{Rep}}
\newcommand{\nnb}{\nonumber}
\newcommand{\lt}{\triangleleft}
\newcommand{\rt}{\triangleright}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZ}{\mathcal{Z}}
\newcommand{\Com}[2]{[ #1, #2 ]}
\newcommand{\ComGrp}[2]{[ #1, #2 ]_{\text{grp}}}
\newcommand{\level}{\operatorname{Lv}}
\newcommand{\code}{\mathcal{C}}


\newcommand{\glosym}[0]{\mathsf{L}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\supp}[1]{\operatorname{Supp}(#1)}
\newcommand{\Ad}{\operatorname{Ad}}
\newcommand{\Irrep}{\operatorname{Irrep}}
\newcommand{\Wt}{\operatorname{Wt}}
\newcommand{\Lin}{\mathfrak{L}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\T}[0]{\mathsf{U}}
\newcommand{\orbit}[1]{O^{\mathcal{T}}(#1)}
\newcommand{\sym}[0]{\overline{S}}
\newcommand{\av}[0]{\mathbb{A}_v}
\newcommand{\bp}[0]{\mathbb{B}_f}
\newcommand{\onsite}[1]{\mathsf{T}|_{#1}}
\newcommand{\Log}[1]{\overline{#1}}
\newcommand{\id}[0]{\mathbf{1}}
\newcommand{\bd}[1]{\delta({#1})}
\newcommand{\zp}[0]{\mathbb{Z}_p}
\newcommand{\cX}[0]{\mathcal{X}}
\newcommand{\cZ}[0]{\mathcal{Z}}
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\cE}[0]{\mathcal{E}}
\newcommand{\cx}[2]{CX_{#1\rightarrow#2}}
\newcommand{\wcp}[2]{\mathcal{C}P_{#1\rightarrow#2}}
\newcommand{\wcx}[2]{\mathcal{C}X_{#1\rightarrow#2}}
\newcommand{\wcz}[2]{\mathcal{C}Z_{#1\rightarrow#2}}
\newcommand{\wcy}[2]{\mathcal{C}Y_{#1\rightarrow#2}}
\newcommand{\cpw}[2]{C\mathcal{P}_{#1\rightarrow#2}}
\newcommand{\cxw}[2]{C\mathcal{X}_{#1\rightarrow#2}}
\newcommand{\czw}[2]{C\mathcal{Z}_{#1\rightarrow#2}}
\newcommand{\cyw}[2]{C\mathcal{Y}_{#1\rightarrow#2}}
\newcommand{\wct}[2]{\mathcal{C}\mathcal{T}_{#1\rightarrow#2}}
\newcommand{\wctdag}[2]{\mathcal{C}\mathcal{T}^\dagger_{#1\rightarrow#2}}
\newcommand{\cnot}[0]{\CNOT}
\newcommand{\SWAP}[0]{\mathsf{SWAP}}
\newcommand{\CNOT}[0]{\mathsf{CNOT}}
\newcommand{\CSWAP}[0]{\mathsf{CSWAP}}
\newcommand{\CX}[0]{\mathsf{CX}}
\newcommand{\CZ}[0]{\mathsf{CZ}}
\newcommand{\CT}[0]{\mathsf{CU}}
\newcommand{\swap}[0]{\SWAP}
\newcommand{\cswap}[0]{\CSWAP}

\newcommand{\overlap}[1]{\Omega(#1)}
\newcommand{\E}[2]{e_{(#1,#2)}}
\newcommand{\dec}[1]{\tilde{#1}}
\newcommand{\insuppof}[2]{#1|_{#2}}
\newcommand{\plushalf}[1]{{#1+\frac{1}{2}}}
\newcommand{\minushalf}[1]{{#1-\frac{1}{2}}}
\newcommand{\scrG}[0]{{\mathscr{G}}}
\newcommand{\sset}[1]{\Sigma(#1)}

\newcommand{\symOP}{\T}
\newcommand{\symS}{\overline{S}}
\newcommand{\haH}{\mathsf{H}}
\newcommand{\haA}{\mathsf{A}}
\newcommand{\haB}{\mathsf{B}}
\newcommand{\haP}{\mathsf{P}}
\newcommand{\haQ}{\mathsf{Q}}
\newcommand{\haX}{\mathsf{X}}
\newcommand{\Deco}{\mathfrak{D}}

\newcommand{\vertexset}[1]{\Sigma^{-1}(#1)}
\newcommand{\invvertexset}[1]{\Sigma(#1)}
\newcommand{\faceP}{\mathcal{P}} 
\newcommand{\vertexV}{\mathsf{V}}
\newcommand{\edgeE}{\mathsf{E}}
\newcommand{\faceF}{\mathsf{F}}
\newcommand{\graphG}{\mathsf{G}}
\newcommand{\intG}{\mathbb{G}}
\newcommand{\N}{\mathsf{N}}
\newcommand{\eigenE}{\mathbf{E}} 
\newcommand{\gaugedA}{\mathbb{A}}
\newcommand{\gaugedB}{\mathbb{B}}
\newcommand{\gaugedS}{\mathbb{S}}
\newcommand{\Sdec}{\mathfrak{s}}
\providecommand{\vr}{}
\renewcommand{\vr}{v_r}
\newcommand{\gaugedH}{\mathbb{H}}
\newcommand{\gaugingOP}{\mathscr{G}}
\newcommand{\chproj}[2]{\llbracket #1\rrbracket _{#2}}

\newcommand{\gX}{\mathcal{X}}
\newcommand{\gZ}{\mathcal{Z}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\gW}{\mathcal{W}}
\newcommand{\gY}{\mathcal{Y}}
\newcommand{\Agrp}{\mathbf{A}}
\newcommand{\chOmega}{\mathit{\Omega}}
\newcommand{\Linex}{\Lin_{\rm ex}(\mathcal H_{\rm m})}
\newcommand{\Linnt}{\Lin_{\rm nt}^{\rm ex}(\mathcal H_{\rm mat})}


\newcommand{\K}{\mathcal{K}}
\newcommand{\gaugedT}{\mathbb{T}}
\newcommand{\Stab}{\mathcal{G}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Hp}{\mathcal{H}}
\newcommand{\Poly}{\mathsf{Poly}}
\newcommand{\Fphys}{F_{\text{phys}}}
\newcommand{\Fmeas}{F_{\text{meas}}}
\newcommand{\Fp}{\mathbf{F}_p}
\newcommand{\Zq}{\mathbb{Z}_q}
\newcommand{\Sprod}[2]{\Lambda\left( #1, #2 \right)}
\newcommand{\FT}{F^T}
\newcommand{\nbhd}{\mathsf{N}}

\newcommand{\Cgeom}{C_{\text{geom}}}
\newcommand{\CLDPC}{C_{\text{LDPC}}}
\newcommand{\Cstep}{C_{\text{step}}}
\newcommand{\Cretract}{C_{\text{retract}}}
\newcommand{\Ctotal}{C_{\text{total}}}
\newcommand{\Cgauge}{C_{\text{gauge}}}

\newcommand{\nonabel}[1]{S^\mathrm{N}_{#1}}
\newcommand{\abel}[1]{S^\mathrm{A}_{#1}}
\newcommand{\gnonabel}[1]{\mathbb{S}^\mathrm{N}_{#1}}
\newcommand{\gabel}[1]{\mathbb{S}^\mathrm{A}_{#1}}
\newcommand{\onset}[2]{{#1}_{\sset{#2}}}
\newcommand{\ccomm}[2]{[#1,#2]_{\mathrm{grp}}}
\newcommand{\tu}[0]{t_{\mathrm{u}}}
\newcommand{\tg}[0]{t_{\mathrm{g}}}
\newcommand{\tf}[0]{t_\mathrm{f}}
\newcommand{\Ig}[0]{\mathrm{I}_{\mathrm{g}}}
\newcommand{\Ifn}[0]{\mathrm{I}_\mathrm{f}}
\newcommand{\Ib}[0]{\mathrm{I}_0}
\newcommand{\cA}[0]{\mathcal{A}}
\newcommand{\cQ}[0]{\mathcal{Q}}
\newcommand{\cK}[0]{\mathcal{K}}
\newcommand{\grpcom}[2]{\ComGrp{#1}{#2}}
\newcommand{\de}[0]{d_\mathcal{E}}



\definecolor{Teal}{RGB}{0,128,128}
\definecolor{Crimson}{RGB}{220,20,60}
\definecolor{RedOrange}{RGB}{255,69,0}
\definecolor{DarkMagenta}{RGB}{139,0,139}
\definecolor{DarkGreen}{RGB}{0,100,0}
\definecolor{MidnightBlue}{RGB}{25,25,112}


\hypersetup{
    colorlinks=true,
    linkcolor=MidnightBlue,
    citecolor=MidnightBlue,
    urlcolor=MidnightBlue,}

\usepackage{amsfonts,latexsym,amsthm,amssymb,amsmath,amscd,euscript,tikz,mathtools}
\usepackage{framed}
\usepackage[normalem]{ulem}
\makeatletter
\@ifclassloaded{revtex4-2}{}{\usepackage[margin=1in]{geometry}}
\makeatother
\usepackage{color}




\usepackage{enumitem}
\usepackage{environ}
\usepackage{dcolumn}

\usetikzlibrary{positioning, shadows, arrows, backgrounds, fit}
\usetikzlibrary{decorations.pathmorphing}

\definecolor{Teal}{RGB}{0,128,128}

\hypersetup{
    colorlinks=true,
    linkcolor=MidnightBlue,
    citecolor=MidnightBlue,
    urlcolor=MidnightBlue,
}

\definecolor{GrayOut}{gray}{0.8}
\NewEnviron{GrayedOut}{\begingroup\color{GrayOut}\BODY\endgroup
}

\newcommand{\diam}{\operatorname{diam}}
\newcommand{\dist}{\operatorname{dist}}

\newcommand{\cH}{\mathcal{H}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\haT}{\mathsf{T}}
\newcommand{\haD}{\mathsf{D}}
\newcommand{\cF}{\mathcal{F}}

\newcommand{\CZero}{C_0(\Gcal_0)}
\newcommand{\COne}{C_1(\Gcal_1)}
\newcommand{\deltaOne}{\delta_1}
\newcommand{\jall}{\mathbf{1}}
\newcommand{\tof}[0]{\ket{\mathsf{Tof}}}
\newcommand{\Pp}[1]{\mathrm{P}^+_{\Log{#1}}}
\newcommand{\Ppk}[1]{\mathrm{P}^+_{\Log{#1}^{\otimes k}}}
\newcommand{\Pm}[1]{\mathrm{P}^-_{\Log{#1}}}

\newcommand{\fa}[0]{F_\mathrm{A}}
\newcommand{\fn}[0]{F_\mathrm{N}}

\newcommand{\CHANGE}[1]{{\color{DarkMagenta}#1}}

\newcommand{\syndromeSet}{\sigma}
\newtheorem{axiom}{Axiom}[section]
\newtheorem{question}{Question}[section]


\newcommand{\green}[1]{\textcolor{Teal}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\makeatletter
\let\UncappedLeft\left
\let\UncappedRight\right
\def\left{\@ifnextchar({\CappedLeftParen}{\UncappedLeft}}
\def\CappedLeftParen(#1\right{\@ifnextchar){\CappedRightParen{#1}}{\UncappedLeft(#1\UncappedRight}}
\def\CappedRightParen#1){\mathopen{}\bigg(#1\bigg)\mathclose{}}
\makeatother

\definecolor{vred}{rgb}{0.85,0,0}
\definecolor{epur}{cmyk}{0.45,0.86,0,0}
\definecolor{poraBase}{cmyk}{0,0.42,1,0}
\colorlet{pora}{poraBase!90!black}
\definecolor{setgray}{RGB}{225,225,225}
\newcommand{\vC}[1]{{\color{vred}#1}}
\newcommand{\eC}[1]{{\color{epur}#1}}
\newcommand{\pC}[1]{{\color{pora}#1}}
\newcommand{\sq}[9]{\left(\begin{smallmatrix}
\vC{#1} & \eC{#2} & \vC{#3}\\[1pt]
\eC{#4} & #5 & \eC{#6}\\[1pt]
\vC{#7} & \eC{#8} & \vC{#9}
\end{smallmatrix}\right)}
\newcommand{\mm}[4]{\begin{smallmatrix}#1 & #2\\ #3 & #4\end{smallmatrix}}
\newcommand{\sqe}[5]{\sq{\cdot}{#1}{\cdot}{#2}{#3}{#4}{\cdot}{#5}{\cdot}}
\newcommand{\Sg}{\mathsf{S}}
\newcommand{\CZbar}{\overline{CZ}}

\setcounter{tocdepth}{1}

